Gaussian Membership Inference Privacy

We propose a novel and practical privacy notion called $f$-Membership Inference Privacy ($f$-MIP), which explicitly considers the capabilities of realistic adversaries under the membership inference attack threat model. Consequently, $f$-MIP offers interpretable privacy guarantees and improved utility (e.g., better classification accuracy). In particular, we derive a parametric family of $f$-MIP guarantees that we refer to as $\mu$-Gaussian Membership Inference Privacy ($\mu$-GMIP) by theoretically analyzing likelihood ratio-based membership inference attacks on stochastic gradient descent (SGD). Our analysis highlights that models trained with standard SGD already offer an elementary level of MIP. Additionally, we show how $f$-MIP can be amplified by adding noise to gradient updates. Our analysis further yields an analytical membership inference attack that offers two distinct advantages over previous approaches. First, unlike existing state-of-the-art attacks that require training hundreds of shadow models, our attack does not require any shadow model. Second, our analytical attack enables straightforward auditing of our privacy notion $f$-MIP. Finally, we quantify how various hyperparameters (e.g., batch size, number of model parameters) and specific data characteristics determine an attacker's ability to accurately infer a point's membership in the training set. We demonstrate the effectiveness of our method on models trained on vision and tabular datasets.

==> 4-definitions.tex <==
\subsection{Membership Inference Attacks from a Hypothesis Testing Perspective}
To protect against Membership Inference Attacks, we will formalize our hypothesis testing perspective.
To do that, we define the following distributions of the algorithm's output
\begin{align}
A_0 &= \mathcal{A}(\mX \cup \left\{\vx\right\}), \text{where } \mX \sim \mathcal{D}^{n-1}, \vx \sim \mathcal{D}\\
A_1(\vx^{\prime}) &= \mathcal{A}(\mX \cup \left\{\vx^{\prime}\right\}), \text{where } \mX \sim \mathcal{D}^{n-1},
\end{align}
where we denote other randomly sampled instances that go into the algorithm by $\mX=\left\{\vx_1, ... \vx_{n-1}\right\}$. Here $A_0$ represents the output distribution under the null hypotheses where the sample $\bx^\prime$ is not part of the training dataset. 
On the other hand, $A_1$ is the output distribution under the alternative hypotheses where $\bx^\prime$ was part of the training dataset.
We observe that the distribution $A_1$ depends on the sample $\vx^{\prime}$ which is known to the attacker. Therefore, the attacker will have access to samples for which $A_0$ and $A_1(\vx^\prime)$ are simpler to distinguish and others where the distinction is harder. To reason about the characteristics of such a stochastically composed test, we define a composition operator that defines an optimal test in such a setup. We note that to obtain a global false positive rate (FPR, type I error) of $\alpha$, an attacker can target different false positive rates $\bar{\alpha}(\vx^{\prime})$ for each specific test. Therefore, we need to consider the optimum over all possible ways of choosing $\bar{\alpha}(\vx^{\prime})$, which we refer to as $\textit{test-specific FPR function}$ and which gives rise to the following definition.
\begin{definition}[Stochastic composition of trade-off functions]
Let 
\begin{itemize}
\setlength{\itemsep}{-3pt}
    \item $\mathcal{F}$ be a family of trade-off functions;
    \item $h: \mathcal{X} \subset \mathbb{R}^d \rightarrow \mathcal{F}$ be a function that maps an instance of the data domain to a corresponding trade-off function;
    \item $\mathcal{D}$ be a probability distribution on $\mathcal{X}$.
\end{itemize}
The set of valid test-specific FPR functions that result in  a global FPR of $\alpha \in [0,1]$ given the distribution $\mathcal{D}$ is given by
\begin{align}
    \mathcal{E}(\alpha, \mathcal{D}) = \left\{\bar{\alpha}: \mathcal{X}\rightarrow \left[0,1\right] ~\middle|~
 \mathbb{E}_{\vx^\prime \sim \mathcal{D}}\left[\bar{\alpha}(\vx^\prime)\right] =\alpha\right\}.
\end{align}
For a given test-specific FPR function $\bar{\alpha}$ the global false negative rate (type II error) $\beta$ is given by 
\begin{align}
    \beta_h(\bar{\alpha}) = \mathbb{E}_{\vx^\prime \sim \mathcal{D}} \left[h(\vx)(\bar{\alpha}(\vx))\right].
\end{align}
where $\bar{\alpha}(\vx)$ is the argument to the trade-off function $h(\vx) \in \mathcal{F}$.
For a global $\alpha \in [0,1]$ the stochastic composition of these trade-functions is defined as
\begin{align}
\left(\bigotimes_{\vx \sim \mathcal{D}} h(\vx) \right)(\alpha) = \min_{\bar{\alpha} \in \mathcal{E}(\alpha, \mathcal{D})} \left\{ \beta_h(\bar{\alpha})\right\},
\end{align}
the smallest global false negative rate possible at a global FPR of $\alpha$.
\end{definition}
This definition characterizes the trade-off function $\bigotimes_{\vx \sim \mathcal{D}} h(\vx): [0,1] \rightarrow [0,1]$ for a stochastic composition of several trade-offs. Below, we show that the stochastic composition has the properties of a standard trade-off function.
\begin{theorem}
The stochastic composition $\bigotimes_{\vx \sim \mathcal{D}} h(\vx)$ of trade-off functions $h(\vx)$ maintains the characteristics of a trade-off function, i.e., it is convex, non-increasing and $\left(\bigotimes_{\vx \sim \mathcal{D}} h(\vx)\right)(r) \leq 1 - r$ for all $r \in [0,1]$.
\end{theorem}
The proof is relegated to \Cref{app_sec:stochasticcomposition}. 

\subsection{$f$-membership Inference Privacy ($f$-MIP)}
This rigorous definition of the stochastic composition operator allows us to define membership inference privacy from a hypothesis testing perspective.
\begin{definition}[$f$-Membership Inference Privacy]
\label{def:f-mip}
Let $f$ be a trade-off
function. An algorithm $\mathcal{A}: D^{n-1} \times D \rightarrow \mathbb{R}^d$ is said to be
$f$-membership inference private ($f$-MIP) with respect to a data distribution $\mathcal{D}$ if
\begin{align}
\bigotimes_{\vx^{\prime} \sim \mathcal{D}}  \text{\normalfont~Test}\left(A_0; A_1(\vx^{\prime}) \right) \geq f,
\end{align}
 where $\vx^{\prime} \sim \mathcal{D}$ and $\bigotimes$ denotes the stochastic composition built from individual trade-off functions of the membership inference hypotheses tests for random draws of $\vx^{\prime}$.
\end{definition}
In this definition, both sides are functions dependent on the false positive rate $\alpha$. A prominent special case of a trade-off function is the Gaussian trade-off, which stems from testing one-dimensional normal distributions of unit variance that are spaced apart by $\mu \in \mathbb{R}_{\geq 0}$. Therefore, defining the following special case of $f$-MIP will be useful.
\begin{definition}[$\mu$-Gaussian Membership Inference Privacy]
\label{def:mu-gmip}
Let $\Phi$ be the cumulative distribution function (CDF) of a standard normal distribution.
Define $g_\mu(\alpha)\coloneqq \Phi(\Phi^{-1}(1-\alpha)-\mu)$ to be the trade-off function derived from testing two Gaussians. 
An algorithm $A$ is $\mu$-Gaussian Membership Inference private ($\mu$-GMIP) with privacy parameter $\mu$ if it is $g_\mu$-MIP, i.e., it is membership inference private with trade-off function $g_\mu$.
\end{definition}

\begin{remark}
Note that Differential Privacy can also be defined via the Gaussian trade-off function, which results in $\mu$-Gaussian Differential Privacy ($\mu$-GDP, \cite{dong2022gaussian}). While the attack trade-off has the same form, the capacities and the target of the attackers are different.
\end{remark}

==> 4-notes-0.tex <==
\subsection{$f$-MIP and one step of DP-SGD}
Here we analyze the susceptibility of one step of DP-SGD to membership inference attacks.
We collect the target model's individual gradients $\vg(\vx_i) \cdot\max\big(1,\frac{C}{\lVert\vg(\vx_i, y_i)\rVert}\big) =\vtheta_i$ in a matrix $\mTheta = [\vtheta_1, \ldots, \vtheta_n]$, where $\vtheta_i \in \mathbb{R}^d$ and $\vtheta_i \sim P$ , where $P$ is any distribution with expected value $\vmu$ and covariance matrix $\mSigma$. 
We follow \citet{abadi2016deep} and make the standard assumption that the mean over the individual gradients $\vm = \frac{1}{n}\sum_{i=1}^n \vtheta_i$ is published.
Consistent with the definition of the membership inference game, $b \in \{0,1\}$ is drawn uniformly at random. 
If $b = 0, \vtheta' \sim \Theta$, else  $\vtheta' \sim P$ and the vector $\vtheta'$ is published.
The adversary has access to $\vm$ and attempts to predict the value of $b$: $\mathcal{A}(\vm, \vtheta')=b'$ , i.e., whether $\vtheta'$ was in the training set or not.
The following hypothesis test succinctly summarizes the adversary's problem in the this setting:
\begin{align}
&H_0: \vtheta' \text{ was drawn from } \mTheta &
&H_1: \vtheta' \text{ was drawn from } P.
\label{eq:hypothesis_test_exact_normal}
\end{align}

We are now interested in determining the shape of the attacker's trade-off function. 
%\textbf{One-step SGD and $g_{\mu}$ membership inference privacy.}
We first consider one step of DP-SGD (i.e., one averaging operation with additional noising, see \Cref{alg:dpsgd}), and establish the following theorem.
\begin{theorem}[One-step DP-SGD is $f$-membership inference private]
Denote the cumulative distribution function of the noncentral chi-squared distribution with $d$ degrees of freedom and non-centrality parameter $\gamma$ by $ F_{\mathcal{X}'^2_d(\gamma)}$. 
Let $K\geq \lVert \mSigma^{-1/2} (\vmu - \vtheta^\prime) \rVert_2^2$ and let $n_{\text{effective}} = n + \frac{\tau^2 n^2}{C^2}$.
Then one step of DP-SGD is $f$-membership inference private with tradeoff function given by:
\begin{align}
\beta(\alpha) = F_{\mathcal{X}'^2_d(n_{\text{effective}}K)}\left(\frac{n_{\text{effective}}}{n_{\text{effective}}-1} F_{\mathcal{X}'^2_d\left((n_{\text{effective}}-1)K\right)}^{-1}(1-\alpha) \right).
\end{align}
\label{theorem:onestep_dp_sgd}
\end{theorem}
%For very few parameters $d$, the above tradeoff curve is distinct in its shape and cannot be converted to the $\epsilon$-DP tradeoff curve \cite{kairouz2015composition}.
% It can however be converted to $\epsilon,\delta$-Differential Privacy with a set of possible $(\epsilon,\delta)$-tuples.
%\begin{wrapfigure}[15]{l}{4.5cm}
%\vspace{-0.75cm}
\begin{figure}
\centering
\begin{subfigure}{0.26\textwidth}
\includegraphics[scale=0.55]{figures/approx_quality_vary_n_d.pdf}
\caption{$\beta$ from Thm.\ \ref{theorem:onestep_dp_sgd} converges to $\tilde{\beta}$ from Coro.\ \ref{corollary:onestep_dp_sgd}.}
\label{fig:vary_n_d}
\end{subfigure}
\hfill
\begin{subfigure}{0.26\textwidth}
\centering
\includegraphics[scale=0.55]{figures/approx_quality_vary_d.pdf}
\caption{Influence of $d$ on the analytical tradeoff curve.}
\label{fig:vary_d}
\end{subfigure}
\hfill
\begin{subfigure}{0.38\textwidth}
\centering
\includegraphics[scale=0.53]{figures/privacy_impact_noise.pdf}
\caption{Influence of noise $\tau^2$ on the analytical privacy level $\mu$ from Corollary \ref{corollary:onestep_dp_sgd}.}
\label{fig:impact_noise}
\end{subfigure}
\caption{\textbf{Illustrating our theoretical results with $n{=}1024$, $\tau^2{=}0$ and $K{=}d$ unless stated o/w}.}
\end{figure}
The larger the number of parameters $d$ and the batch size $n$ grow, the more the trade-off curve approaches the $\mu$-GMIP curve, which we show next (see also Figure \ref{fig:vary_n_d}).
\begin{corollary}[One step DP-SGD is approx.\ GMIP.]
For large large $d,n$, DP-SGD is approximately $g_\mu$-GMIP. In particular, $\beta(\alpha) \approx \tilde{\beta}(\alpha) = \Phi(\Phi^{-1}(1-\alpha)-\mu)$ with privacy parameter:
\begin{align}
\mu = \frac{d + (2n_{\text{effective}} - 1) K }{n_{\text{effective}} \sqrt{2d + 4 n_{\text{effective}} K}}.
\end{align} 
\label{corollary:onestep_dp_sgd}
\end{corollary}
% \begin{figure}
% \centering
% \includegraphics[scale=0.5]{figures/impact_noisy.pdf}
% \caption{Effect of noise on privacy level $\mu$ in Large Models when $K=10$.}
% \label{fig:effect_of_noise_on_large_models}
% \end{figure}
% \begin{corollary}
% For large $d,n$, SGD is approximately $g_\mu$-GMIP. In particular, $\beta(\alpha) \approx \tilde{\beta} (\alpha) =  \Phi(\Phi^{-1}(1-\alpha)-\mu)$ with privacy parameter:
% \begin{align}
% \mu = \frac{d + (2n - 1) K }{n\sqrt{2d + 4 n K} }.
% \end{align} 
% \label{theorem:onestep_cropped_sgd}
% \end{corollary}
\begin{hproof}
% The proof for Theorem \ref{theorem:onestep_dp_sgd} and Corollary \ref{corollary:onestep_dp_sgd} follows two steps:
% We establish the hardness of the individual tests using the Neyman-Person lemma.
% Then, we establish that the chi squared tradeoff curve for large $n, d$ follows the tradeoff-curve $\mu_g$.
% We then use a lower bound on the stochastic composition provided in \Cref{app_thm:worstcasestoasticcomp}.
Based on the above hypothesis testing setup, the adversary uses the Neyman-Pearson Lemma to construct a likelihood ratio test. 
Here we briefly summarize the individual proof steps:
First, we derive the distributions of $\vm$ under the null and the alternative hypothesis.
Second, given these two distributions, we can setup the likelihood ratio, which will yield the test statistic $S=\left(\vm-\vtheta'\right)^\top\mSigma^{-1}\left(\vm-\vtheta'\right)$. 
Third, given the test statistic $S$ and the distribution under the null hypothesis, we derive the rejection region of the likelihood ratio test for a given level $\alpha$. Given the rejection region, we derive the false negative rate $\beta(\alpha)$ of the likelihood ratio test. 
This trade-off function depends on the CDF and inverse CDF of the non-central $\chi^2$ distribution. 
In a final step, we provide approximations to the trade-off function for large $d,n$.
\end{hproof}
We see that the trade-off function depends on four factors: the batch size $n$, the number of parameters $d$, the strength of the noise $\tau^2$ and the data-dependent \emph{gradient susceptibility} $\lVert \mSigma^{-1/2} (\vmu - \vtheta^\prime) \rVert_2^2$.
Intuitively, the ratio of $d$ to $n$ determines how close the tradeoff function is to the diagonal, which is equivalent to having the adversary randomly guess whether a gradient $\vtheta'$ was part of the training data or not. 
The higher $d$ is relative to $n$, the easier it is for the adversary to identify training data points (see Figure \ref{fig:vary_d}). 
Further, everything else constant, the higher the gradient susceptibility which is a measure of the atypicality of a sample with respect the distribution. The higher the susceptiblity term, the more likely will membership inference attacks succeed in identifying training data membership. Unfortunately, if we do not wish to restrict the gradient distribution or its support such a cutoff is unavoidable, as there might always exist samples that distort the mean so drastically that there membership in the training dataset will be given away. This is similar to the $\delta$ parameter in differential privacy, which also permits certain exceptions for exceedingly unlikely events. However, we are able to make the following two remarks about the magnitude of the gradient susceptibility term $K$.
% In the usual SGD-regime, where the number of parameters $d$ is much larger than the batch size $n$ (i.e., $d \gg n, K$) we obtain $\mu \in \mathcal{O}\left(\frac{\sqrt{2d}}{n_{\text{effective}}}\right)$.
% On the other hand, in the regime of large batch sizes (i.e., $n \gg K, d$) we obtain $\mu \in \mathcal{O}\left(\sqrt{\frac{K}{n_{\text{effective}}}} \right)$.
% In the usual SGD-regime we have that $d \gg n, K$; and therefore we obtain $\mu_{\text{MIP}}\in \mathcal{O}\left(\frac{\sqrt{2d}}{n}\right)$.
% On the other hand, in the regime of large batch sizes we have that $n \gg K, d$; and therefore we obtain $\mu_{\text{MIP}} \in \mathcal{O}\left(\sqrt{\frac{K}{n}} \right)$.
% Finally, note that a higher $K$ always leads to less privacy:
% \begin{align}
%  \frac{\partial \mu_{\text{MIP}}}{\partial K} > 0, ~\forall n \geq 1, k \geq 0.
% \end{align}

\begin{remark}
When the dimensions of the uncorrelated components in $\mSigma^{-\frac{1}{2}}(\vmu-\vtheta')$ are also independent, we expect $K$ to follow a $\chi^2$-distribution with $d$ degrees of freedoms and thus $K \in \mathcal{O}(d)$. In the usual SGD-regimes where $d, n \gg 1$, we then obtain $\mu \in \mathcal{O}(\sqrt\frac{d}{n_{\text{effective}}})$.
% In the usual SGD-regime, where the number of parameters $d$ is much larger than the batch size $n$ (i.e., $d \gg n, K$) we obtain $\mu \in \mathcal{O}\big(\frac{\sqrt{2d}}{n_{\text{effective}}}\big)$.
% On the other hand, in the regime of large batch sizes (i.e., $n \gg K, d$) we obtain $\mu \in \mathcal{O}\big(\sqrt{\frac{K}{n_{\text{effective}}}} \big)$.
\end{remark}

\begin{remark}
Note that it is possible to derive an upper bound of the probability of $P(\lVert \mSigma^{-1/2} (\vmu - \vc) \rVert_2^2 \geq K) \leq \frac{d}{K}$ using the Markov bound for general distributions. In the independent regime, $\lVert \mSigma^{-1/2} (\vmu - \vc) \rVert_2^2 \sim \chi_2(d)$ which has a tail bound of $P(\lVert \mSigma^{-1/2} (\vmu - \vc) \rVert_2^2 \geq K) \leq \exp\left(-\frac{K}{20}\right)$ for $K\geq2d$.
\end{remark} 

% For small values of $d$, the tradeoff curve is distinct in its shape and cannot be converted to 
%the pure $\epsilon$-DP tradeoff curve \cite{kairouz2015composition} or to 
% $\mu$-GMIP.
%It can however be converted to $\epsilon,\delta$-Differential Privacy with a set of possible $(\epsilon,\delta)$-tuples.
% On the other hand, for larger sets of parameters $d$, the curve approaches the $\mu$-GMIP curve. %, which we will show next.
%https://math.stackexchange.com/questions/2864188/chi-squared-distribution-tail-bound
% Todo: write down proves.

% \textbf{One-step DP-SGD and $\mu_{\text{MIP}}$--privacy.}

% Compared to the setup before, this time we add Gaussian noise to the published gradients: $\tilde{\vm} = \frac{1}{n}\sum_{i=1}^n \vtheta_i + Y$, where  $Y \sim \mathcal{N}(\mathbf{0}, \tau^2\mI)$.

%In this case, one can show that the following test statistic can be crafted by the adversary to be able to maximally distinguishe gradients from the training set from gradients from the test set; it leads to the highest power (i.e., $1-\beta(\alpha)$) for any fixed false-positive rate (i.e., $\alpha$):
% \begin{align}
% S = \left(\tilde{\vm}-\vx^{'}\right)^\top\mSigma^{-1}\left(\tilde{\vm}-\vx^{'}\right).
% \end{align}
%\subsection{One SGD-step and $\mu_{\text{MIP}}$--privacy}
% \begin{corollary}[MIP of one-step DP-SGD]
% Let $K\geq \lVert \mSigma^{-1/2} (\vmu - \vc) \rVert_2^2$. For large $d,n$, DP-SGD is $g_\mu$-MIP with privacy parameter
% \begin{align}
% \mu = \frac{d + \big(2n_{\text{effective}} - 1\big) K }{n_{\text{effective}}\sqrt{2d + 4 n_{\text{effective}} K }},
% \end{align}
% where $n_{\text{effective}} = n + \frac{\tau^2 n^2}{C^2}$.
% \label{theorem:onestep_dp_sgd}
% \end{corollary}
% In the usual SGD-regime, where the number of parameters $d$ is much larger than the batch size $n$ (i.e., $d \gg n, K$) we obtain $\mu \in \mathcal{O}\left(\frac{\sqrt{2d}}{n_{\text{effective}}}\right)$.
% On the other hand, in the regime of large batch sizes (i.e., $n \gg K, d$) we obtain $\mu \in \mathcal{O}\left(\sqrt{\frac{K}{n_{\text{effective}}}} \right)$.

% This section contains the first formal results
\subsection{Composition and Subsampling}
\label{sec:composition}
In the previous Section we have derived the trade-off function for one step of DP-SGD. 
Since DP-SGD is run over multiple rounds, we require an understanding of how the individual trade-off functions can be composed when a sequence of $f$-MIP operations is conducted and a random subset of the entire data distribution is used as an input for the privatized algorithm.
The next lemma provides such a result for $\mu$-GMIP and follows from a result that holds for general privacy notions that can be written as hypotheses tests due to Dong et al. \cite{dong2022gaussian} (see \Cref{sec:app_compositionresults} for details).
% \begin{lemma}[Composition theorem for $\mu$-MIP]
% The $n$-fold composition of $\mu_i$-MIP mechanisms is $\sqrt{\mu_1^2 + \ldots + \mu_n^2}$-MIP.
% \end{lemma}
% \begin{proof}
% \citet{dong2022gaussian}, Corollary 3.3.
% \end{proof} 

% Thus, when performing $r$ iterations of DP-SGP with a target of $\mu_{\text{total}}$, the individual steps require a privacy level of $\frac{\mu_\text{total}}{\sqrt{r}}$ because 
% $\sqrt{r\left(\frac{\mu_{\text{total}}}{\sqrt{r}}\right)^2} = \sqrt{r\frac{\mu_{\text{total}}^2}{r}} = \mu_\text{total}$.

\begin{lemma}[Asymptotic convergence of DP-SGD]
Let $n$ be the batch size in SGD, $T$ be the number of iterations and $N$ be the entire size of the dataset. If a single SGD-Step is at least as hard as $\mu_{\text{step}}$-MIP with respect to the samples that were part of the batch and $\frac{n\sqrt{t}}{N} \rightarrow c$ as $\lim_{t\rightarrow \infty}$, then the private-SGD algorithm will be $\mu$-MIP with \begin{align}
    \mu = \sqrt{2} c\sqrt{\exp(\mu_{\text{step}}^2) \Phi\left(\frac{3}{2}\mu_{\text{step}}\right) + 3\Phi\left(-\frac{1}{2}\mu_{\text{step}}\right)-2}.\label{eqn:dongfactor}
\end{align}
\label{lem:composition}
\end{lemma}
Note that this result also provides a (loose) bound on the case where exactly $T$ iterations with a batch size of $n^\prime$ with $c=\frac{n^\prime\sqrt{T}}{N}$ (through using $n(t)=n^\prime~\text{if}~t\leq T,~\text{else}~n(t) = \frac{n^\prime\sqrt{T}}{\sqrt{t}}$). With this result in place, we are able to defend against membership inference attacks using the standard DP-SGD algorithm. 
% Asymptotics. For $\mu_{\text{step}} \approx 0$ and $\frac{\partial\Phi(x)}{x}(0) = \frac{1}{\sqrt{2\pi}}$ and thus 
% \begin{align}\mu &\approx \sqrt{2} c\sqrt{\exp(\mu_{\text{step}}^2) \left(0.5+\frac{1}{\sqrt{2\pi}}\frac{3}{2}\mu_{\text{step}}\right) + 3\left(0.5-\frac{1}{\sqrt{2\pi}}\frac{1}{2}\mu_{\text{step}}\right)-2}\\
% &= \sqrt{2} c\sqrt{\frac{1}{2}\left(\exp(\mu_{\text{step}}^2) -1\right) +\frac{1}{\sqrt{2\pi}}\frac{3}{2}\left(\exp(\mu_{\text{step}}^2)-1\right)}\\
% &= \sqrt{2} c\sqrt{\left(\exp(\mu_{\text{step}}^2) -1\right)}\sqrt{\frac{1}{2} +\frac{1}{\sqrt{2\pi}}\frac{3}{2}\mu_{\text{step}}}\\
% &=c\sqrt{\left(\exp(\mu_{\text{step}}^2) -1\right)}\sqrt{1+\frac{3}{\sqrt{2\pi}}\mu_{\text{step}}}\\
% &\approx c \mu_{\text{step}}
% \end{align}

% We can use this results to form a guaranteed for SGD with fixed batch size as well.
% \begin{corollary}
%     Performing $T$ iterations of Noisy SGD with a fixed batch size of $n$, a dataset size of $N$ will be $\mu$-GMIP with 
%     \begin{align}
%         \mu = \sqrt{2} \frac{n\sqrt{T}}{N}\sqrt{\exp(\mu_{\text{step}}^2) \Phi\left(\frac{3}{2}\mu_{\text{step}}\right) + 3\Phi\left(-\frac{1}{2}\mu_{\text{step}}\right)-2} \approx  \frac{n\sqrt{T}}{N}\mu_{\text{step}},
%     \end{align}
%     where $\mu_{\text{step}}=\frac{d + (2n_{\text{effective}} - 1) K }{n_{\text{effective}}\sqrt{2d + 4 n_{\text{effective}} K }}$ is the privacy level of a single step.
% \end{corollary}

% \begin{lemma}
% The tradeoff curve for testing two Gaussian distributions $\mathcal{N}\left(\vmu_1, \sigma^2_1 \mI\right)$ vs $\mathcal{N}\left(\vmu_2, \sigma^2_2 \mI\right)$ is given by
% \begin{align}
% \text{Test}\left(\mathcal{N}\left(\vmu_1, \sigma^2_1 \mI\right), \mathcal{N}\left(\vmu_2, \sigma^2_2 \mI\right)\right) = \Phi\left(\frac{\sigma_1}{\sigma_2}\Phi^{-1}(1-\alpha)-\frac{1}{\sigma_2}\lVert\vmu_2-\vmu_1\rVert_2\right)
% \end{align}
% \end{lemma}
% \textbf{Proof.}
% An optimal test statistic for testing $\vx$ would be $S=\frac{\vx^\top(\vmu_2-\vmu_1)}{\lVert\vmu_2-\vmu_1\rVert_2}$
% The problem can be reduced to $\text{Test}\left[\mathcal{N}\left(0, \sigma_1^2\right), \mathcal{N}\left(\lVert\vmu_2-\vmu_1\rVert_2, \sigma_2^2\right)\right]$ and to  $\text{Test}\left[\mathcal{N}\left(0, 1\right), \mathcal{N}\left(\frac{\lVert\vmu_2-\vmu_1\rVert_2}{\sigma_1}, \frac{\sigma_2^2}{\sigma_1^2}\right)\right]$.
% The tradeoff function for this test is
% \begin{align}
% \text{Test}\left(\mathcal{N}\left(\vmu_1, \sigma^2_1 \mI\right), \mathcal{N}\left(\vmu_2, \sigma^2_2 \mI\right)\right) &= \Phi\left(\frac{\Phi^{-1}(1-\alpha)\sigma_1-\frac{\lVert\vmu_2-\vmu_1\rVert_2}{\sigma_1}\sigma_1}{\sigma_2}\right)\\
% &= \Phi\left(\frac{\sigma_1}{\sigma_2}\Phi^{-1}(1-\alpha)-\lVert\vmu_2-\vmu_1\rVert_2\frac{1}{\sigma_2}\right)
% \end{align}
% For instance, we can compare 
% Let $P = C$, than sensitivity is $\frac{C}{n}$.

==> 4-notes-1.tex <==
\subsection{Intro into Hypothesis Testing}
A test statistic $T$ is any statistic such that extreme values (large or small) of $T$ provide evidence against $H_0$.
When devising a hypothesis test for testing $H_0$ against $H_1$, we face the following optimization problem:
\begin{itemize}
    \item[(1)] \textbf{Maximize}: The power of the test against $H_1$
    \item[(2)] \textbf{S.t.}: The significance level of the test under the null hypothesis $H_0$ is at most $\alpha$
\end{itemize}

\subsection{The Loss-based Test}
\paragraph{Form of the test}
Denote by $\mathcal{D}$ the data domain. 
Denote by $\mathcal{D}_{\text{Train}} = \{(\mX_i, y_i)\}_{i=1}^n \subset \mathcal{D}$ the training data set used to train the predictive model $g_{\btheta}: \mathbb{R}^d \to \mathbb{R}$ which is parameterized by $\btheta$.
We require that there are no duplicate tuples $(\mX_i, y_i)$ within the data set.
The model parameters are usually obtained by solving the empirical risk minimization problem:
\begin{align}
\btheta(\mathcal{D}_{\text{Train}}) = \argmin_{\btheta'} \sum_{i \in \mathcal{D}_{\text{Train}}} \ell(y_i, g_{\btheta'}(\mX_i)).
\end{align}
Usually, we will drop the dependence of $\btheta$ on $\mathcal{D}_{\text{Train}}$ from the notation to avoid clutter.
In the membership inference attack literature, for a query instance $\bz'=(\mX',y')$, the standard hypothesis test takes the following form:
\begin{align}
\texttt{predict}(\bz_1', \btheta) =
\begin{cases}
\text{train} & \text{ if } T = \ell(\bz_1', \btheta) < \gamma  \\
\text{test} & \text{ else},
\end{cases}
\end{align}
where $\btheta$ are the estimated model parameters.

As opposed to the above testing procedure, for the LRT, we will be interested in the following hypotheses:
\begin{align}
\text{H}_0: \bz'= (\mX',y') \in \mathcal{D}_{train}  \text{ vs } \text{H}_1: \bz'=(\mX',y') \not \in \mathcal{D}_{train}. 
\label{eq:hypotheses}
\end{align}

\paragraph{The Model}
Before, we will do the analysis, let us take a look at the model assumptions.
Let $\by$ be the observed labels. 
The presence of additive label noise corrupts the true labels such that:
\begin{align}
\mathbf{y} = \mathbf{f}(\mX) + \vm{\varepsilon} = \mX \bbeta  + \vm{\varepsilon}, && \vm{\varepsilon} \sim \mathcal{N}(\mathbf{0}, \sigma^2 \mathbf{I}_n),
\label{eq:model_assumption}
\end{align}
where $\mathbf{f} \in \mathbb{R}^n$ denotes the true underlying targets, and where $\bbeta$ are the population (i.e., true) model parameters.
In modern ML theory literature, the above model is sometimes called a ``teacher model''.
Note that the above model assumption amounts to assuming the following data generating process: 
\begin{align}
p(y|f(\mX), \sigma^2) = \mathcal{N}(f(\mX), \sigma^2).
\end{align}
Note that this is a standard model in many undergraduate and graduate ML and statistics text books.
For now, let $g_{\btheta}(\mX) = \mX^\top \btheta$ denote our model output.
In case of linear regression, we solve the empirical risk minimization problem using the mean-squared-error (MSE) loss:
\begin{align}
\begin{split}
\btheta &= \argmin_{\btheta'} \sum_{i=1}^n (y_i - \btheta'^\top \mX_i)^2 \\
      &= (\mX^\top \mX)^{-1} \mX^\top \mathbf{y} \\
      &= \underset{Signal}{(\mX^\top \mX)^{-1} \mX^\top \mX \bbeta} + \underset{Noise}{(\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}} ,
\end{split}
\end{align}
where $\mX \in \mathbb{R}^{n \times (d+1)}$ and $\mathbf{y} \in \mathbb{R}^n$ are the training instances and training labels, respectively.\footnote{As long as the noise is normal and linear in the ``noise term'' we should be able to conduct this kind of analysis.}
Moreover, by the above model stated in \eqref{eq:model_assumption} it can be shown that, for fixed $\mX$, $\btheta$ is a random variable which follows a normal distribution:
\begin{align}
\btheta \sim \mathcal{N}(\bbeta, \mH),
\end{align}
where we have computed the expectations and variances as follows:
\begin{align}
\mathbb{E}_{\varepsilon}[\btheta|\mX] &= \mathbb{E}_{\varepsilon}[(\mX^\top \mX)^{-1} \mX^\top \mathbf{y}|\mX] \\
&= \mathbb{E}_{\varepsilon}[(\mX^\top \mX)^{-1} \mX^\top \mX \bbeta|\mX] + \mathbb{E}_{\varepsilon}[(\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}|\mX] \\
&= \bbeta \\
\mathbb{V}_{\varepsilon}[\btheta|\mX] &= \mathbb{V}_{\varepsilon}[(\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}|\mX] \\
&= (\mX^\top \mX)^{-1} \mX^\top \mathbb{V}_{\varepsilon}[\vm{\varepsilon}|\mX] \big((\mX^\top \mX)^{-1} \mX^\top\big)^\top \\
&= \sigma^2 (\mX^\top \mX)^{-1} \\
&= \mH
\end{align}
where we leveraged the model setup in \eqref{eq:model_assumption} for the second-to-last display, i.e., $\mathbb{V}_{\varepsilon}[\vm{\varepsilon}|\mX] = \sigma^2 \mI$. It can also be easily verified that $\mH$ is proportional to the Hessian of the MSE loss with respect to $\bbeta$.
We now have all the ingredients to state our main result.

\paragraph{The Information Sets, the Inference Game and the Identification Strategy}
\begin{itemize}
\item[\textbf{Principal}] Following the standard in the literature, we assume that the principal makes the first move. 
She draws a training data set $\mathcal{D}_{\text{Train}}$, and fits a model  $g_{\btheta}: \mathbb{R}^d \to \mathbb{R}$ using the training data set. 
As a consequence, the model parameters ${\btheta}$ and the training data set $(\mX, \by)$ are now fixed.
\item[\textbf{Adversary}] The adversary obtains a sample $\bz_1'=(\mX_1', y_1')$ which could either be from the train or test set. For the purpose of the analysis we also assume that the adversary knows that a linear model with Gaussian label noise as postulated in \eqref{eq:model_assumption} will be fit.
% \item[\textbf{Identification}] The underlying idea is the following: under the alternative hypothesis, a sample $\bz_1' = (\mX_1', y_1')$ is ``uniquely encoded'' by its label noise $\varepsilon_1'$ since $y_1' = f(\mX_1') + \varepsilon_1'$.
% Why is that? Recall that the estimator $\btheta$ is a function of the training data, \emph{including the label noise} (to see this recall that $\btheta(\vm{\varepsilon},\bbeta, \mX) = (\mX^\top \mX)^{-1} \mX^\top \by = (\mX^\top \mX)^{-1} X^\top \bbeta +  (\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}$).
% When computing the loss $\ell(\bz_1'; \btheta) = y_1' - \btheta^\top \mX_1'$, the (population) mean loss will be the same whether we are under the alternative or null hypothesis\footnote{This is the case since $\btheta$ is an unbiased estimator of $\bbeta$.}, but the (population) variances are different since the label $y_1'(\varepsilon_1')=f(\mX'_1) + \varepsilon_1'$ from $\bz_1'=(\mX_1', y_1') =(\mX_1', f(\mX_1') + \varepsilon_1') = \bz_1 = (\mX_1, f(\mX_1) + \varepsilon_1) \in \mathcal{D}_{\text{train}}$ will covary with the random variable $\btheta(\varepsilon_1)$, while the label from $\bz_1' \not \in \mathcal{D}_{\text{train}}$ will not. See figure \ref{fig:my_label} for an example of the resulting loss distributions when $\bz'_1$ is a training data point versus when it is not.
% To see this more clearly, compute the following covariances:
% \begin{align}
% \mathbb{C}_{\varepsilon}[y'_1, \btheta|\mX, \bz_1' \in \mathcal{D}_{\text{Train}}] = \mathbb{C}_{\varepsilon}[y'_1, \mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}|\mX, \bz_1' \in \mathcal{D}_{\text{Train}}] \neq 0  \\
% \mathbb{C}_{\varepsilon}[y'_1, \btheta|\mX, \bz_1' \not \in \mathcal{D}_{\text{Train}}] = \mathbb{C}_{\varepsilon}[y'_1, \mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}|\mX, \bz_1' \not \in \mathcal{D}_{\text{Train}}] = 0.
% \end{align}
\end{itemize}



% \begin{theorem}
% Consider the model from \eqref{eq:model_assumption}. For a given query instance $\bz_1'=(\mX_1',y_1')$, consider the loss-based statistic $\ell(\btheta, \bz_1')=(y_1' - \btheta^\top \mX_1')$ to construct a test against $H_1$. 
% At fixed false-positive-rate $\alpha$, the optimal threshold rule $\gamma^*$ for the most powerful test to reject the null hypothesis in favour of the alternative when the alternative hypothesis is true is given by:
% \begin{align}
%     \ell^2(\btheta, \bz_1')\leq  \gamma^*,
% \end{align}
% where $\gamma^* = v_0 \text{CDF}_{\mathcal{X}^2}^{-1}(\alpha)$ with $v_0 = \sigma^2 \big(1 + \mX_1'^\top \big( \mX^\top \mX\big)^{-1}  \mX_1' \big)$.
% Further, the statistical power of the test is given by:
% \begin{align}
%     p_{\text{TPR}} = \text{CDF}_{\mathcal{X}^2_1}\bigg(\frac{v_0}{v_1} \text{CDF}_{\mathcal{X}^2_1}^{-1} \big(\alpha \big)\bigg),
% \end{align}
% where $v_1=\sigma^2 \big(1 - \mX_1'^\top \big( \mX^\top \mX\big)^{-1}  \mX_1' \big)$.
% \end{theorem}

% \paragraph{Comments} Some remarks are in place: First of all, this result shows that MI attacks are possible even when the underlying model is linear. 
% This goes against conventional wisdom, which suggests that models have to be overfit for MI attacks to work.
% \begin{itemize}
%     \item[\textbf{On power \& size}] In practice, one often chooses a significance level $\alpha \in \{0.001, 0.01, 0.05\}$. The lower the significance level, the higher $v_0$ (i.e., the variance of the loss under the null hypothesis) has to be to increase the power of the test. In particular, if the leverage of a point $\mX$ is high, then $v_1$ will be much lower than $v_0$, and the power of the test will be high.
    
%     \item[\textbf{Identification}] Note that the identifying information for the test comes from the label noise, which allowed us to determine the distribution of the loss under both the null and the alternative hypotheses. Can we relax this assumption?
    
%     \item[\textbf{Relation to Leverage}] Note that the power of test depends on $\mX^\top (\mX^\top \mX)^{-1} \mX$ under both the null and the alternative hypothesis. This term is proportional to a term that is called \textbf{leverage} in the statistics literature (i.e., $L_x = \mX^\top (\mX^\top \mX)^{-1} \mX$). Intuitively, in a linear model, it measures how the predicted target $\hat{y} = \mX^\top \btheta = \mX^\top (\mX^\top \mX)^{-1} \mX y$ changes as we change the true label $y$, i.e., $\frac{\partial \hat{y}}{\partial y}$.
    
%     \item[\textbf{Making it practical}] At a fixed FPR, the optimal decision rule only depends on the leverage score under the null hypothesis, and the general noise level $\sigma^2$. For practical purposes, both can be estimated. First, the Hessian can be estimated by zero-order methods\footnote{E.g., see \url{https://arxiv.org/pdf/1812.11377.pdf} and \url{https://arxiv.org/pdf/2205.14737.pdf}}; while the general noise level can be estimated using using the shadow data set $\{(y_j, \mX_j)\}_{i=1}^m$ and query access to $g_{\btheta}$: $\sigma^2 \approx \frac{1}{m-1}\sum_{j=1}^m \hat{\varepsilon}^2 = \frac{1}{m-1} \sum_{j=1}^m (y_j -g_{\btheta}(\mX_j))$.
% \end{itemize}
% Next, we provide a proof of the claimed result.

% \begin{hproof}
% Under the model in \eqref{eq:model_assumption}, we first derive the distribution of $(y_1' - \btheta^\top \mX_1')$ under both the null and alternative hypotheses. 
% We show that under the null and alternative hypotheses, these distributions follow Gaussians with mean $0$ and different variances that depend on whether the null or the alternative distribution are true.
% We then use facts about the relation of Gaussian and Chi-squared random variables to find the distribution $(y_1' - \btheta^\top \mX_1')^2$ under the null and the alternative hypotheses.
% Finally, using these insights, we construct the likelihood-ratio.
% \end{hproof}


% \begin{remark}
% Clearly, computing the threshold is not feasible as it depends on the true noise variance $\sigma^2$, the true training point $x_1$, and the covariance matrix / Hessian $H$.
% \end{remark}

% \begin{remark}
% Usually a hypothesis test works like this: we know the (approximate) distribution of the test-statistic when the null hypothesis is true. 
% When the test-statistic is large, we reject the null; and conclude that the alternative is more likely.
% In our setup, the issue is this: the distribution of the loss $(y_1' - \btheta^\top \mX_1')$ is centered around 0 and we want to make conclusion when the test statistic is close to 0 as opposed to small (i.e, negative).
% %\textbf{What does this tell us?}
% % It suggests that thresholding on the loss (i.e., when loss is small $\xrightarrow{}$ conclude TRAIN) is a ``non-membership'' inference attack as low losses are likely to occur under both the null and alternative hypotheses and large losses are more likely to be from non-training samples.
% % This also suggests to construct the threshold using the distribution under the alternative as it is more informative. 
% % However, this is infeasible as it clearly depends on the true training point $x_1$.
% \end{remark}


% \begin{figure}
% \centering
% \pgfmathdeclarefunction{gauss}{2}{%
%   \pgfmathparse{1/(#2*sqrt(2*pi))*exp(-((x-#1)^2)/(2*#2^2))}%
% }
% \begin{tikzpicture}
% \begin{axis}[
%   no markers, domain=-6:6, samples=100,
%   axis lines*=left, xlabel=$(y_1' - \btheta^\top \mX_1')$, ylabel=$p(y_1' - \btheta^\top \mX_1')$,
%   every axis y label/.style={at=(current axis.above origin),anchor=south},
%   every axis x label/.style={at=(current axis.right of origin),anchor=west},
%   height=5cm, width=12cm,
%   xtick={0,6.5}, ytick=\empty,
%   enlargelimits=false, clip=false, axis on top,
%   grid = major
%   ]
%   \addplot [fill=red!20, draw=none, domain=3.5:5.96] {gauss(0,2)} \closedcycle;
%   \addplot [fill=red!20, draw=none, domain=-3.5:-5.96] {gauss(0,2)} \closedcycle;

%   \addplot [very thick,red!50!black] {gauss(0,2)};
%   \addplot [very thick,cyan!50!black] {gauss(0,1)};

% %\draw [yshift=-0.6cm, latex-latex](axis cs:4,0) -- node [fill=white] {$1.96\sigma$} (axis cs:5.96,0);
% \end{axis}
% \end{tikzpicture}

% \caption{
% Density functions of $y_1' - \btheta^\top \mX_1'$ under the \textcolor{red}{null hypothesis} and the \textcolor{blue}{alternative hypothesis}. The distribution under the alternative hypothesis depends on the true training sample $x_1$, which is unknown to the adversary at inference time.}
% \label{fig:my_label}
% \end{figure}

\subsection{Proof of Likelihood Ratio Test}

\begin{proof}
Our goal will be to find the distribution of $(y_1' - \btheta^\top \mX_1')^2$ under both the null and the alternative hypotheses in order to construct the likelihood ratio test. 

\paragraph{The Likelihood Ratio in Favour of $H_1$}
We will reject the null hypothesis in favour of the alternative hypothesis, if:
\begin{align}
\Lambda_{Loss} = \frac{p_1\big(\ell\big(\btheta(\mathcal{D}_{train}), \bz_1'\big)\big| \bz_1' \not \in \mathcal{D}_{train} \big)}{p_0\big(\ell(\btheta(\mathcal{D}_{train}), \bz_1'\big) \big| \bz_1' \in \mathcal{D}_{train}\big)} > \tau.
\end{align}

\paragraph{Deriving the Densities under $H_0$ and $H_1$}
As a direct consequence of our model setup in \eqref{eq:model_assumption} we obtain:
\begin{align}
    y_1' \sim \mathcal{N}(\bbeta^\top \mX_1', \sigma^2).
\end{align}
From well-known facts about Gaussian random variables we have:
\begin{align}
  \hat{y}_1 = \btheta^\top \mX_1' \sim \mathcal{N}(\bbeta^\top \mX_1', \mX_1'^\top \mH \mX_1'). %= \mathcal{N}\big(\bbeta^\top \mX_1', \frac{\partial \hat{y}_1}{\partial y_1'} \big) .
\end{align}
As a consequence, we have:
\begin{align}
y_1' - \btheta^\top \mX_1' \sim \mathcal{N}\big(0, \sigma^2 + \mX_1'^\top \mH \mX_1' - 2 \cdot \mathbb{C}(y_1', \btheta^\top \mX_1'|\mX) \big),
\end{align}
where we have used that:
\begin{align*}
\mathbb{V}( y_1' - \btheta^\top \mX_1'|\mX) &= \mathbb{V}(y_1'|\mX) + \mathbb{V}(\btheta^\top \mX_1'|\mX)  + 2 \cdot \mathbb{C}( y_1', - \btheta^\top \mX_1'|\mX) \\
&= \mathbb{V}(y_1'|\mX) + \mathbb{V}(\btheta^\top \mX_1'|\mX)  - 2 \cdot \mathbb{C}( y_1', \btheta^\top \mX_1'|\mX) \\
\mathbb{V}(y_1'|\mX) &= \mathbb{V}(x_1^\top \bbeta + \varepsilon_1|\mX) = \mathbb{V}(\varepsilon_1|\mX) = \sigma^2 \tag{Since $\mX_1$ and $\bbeta$ are constant} \\
\mathbb{V}(\btheta^\top \mX_1'|\mX) &= \mX_1'^\top  \mathbb{V}(\btheta|\mX) \mX_1' =\mX_1'^\top \mH \mX_1'.
\end{align*}
It remains to determine the form of the covariance $\mathbb{C}(y_1', \btheta^\top \mX_1'|\mX)$.
Next, first we note that $\varepsilon_i$ is independent of $\varepsilon_j$ for all $i \neq j$. Therefore, it suffices to focus on the diagonal terms:
\begin{align}
\mathbb{C}(y_1', \btheta^\top \mX_1'|\mX) & = \mathbb{C}(x_1^\top \bbeta + \varepsilon_1, \btheta^\top \mX_1'|\mX) =  \mathbb{C}(\varepsilon_1', \btheta^\top \mX_1'|\mX) \tag{Since $\mX_1$ and $\bbeta$ are constant} \\
& = \mathbb{C}(\varepsilon_1',  \mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \mX \bbeta + \mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}|\mX) \\
& = \mathbb{C}(\varepsilon_1', \mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}|\mX) \tag{Since $\mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \mX \bbeta$ is constant} \\
& =  \mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \mathbb{C}(\varepsilon_1',\vm{\varepsilon}|\mX) \\
&= \mX_1'^\top (\mX^\top \mX)^{-1} \mX_1 \mathbb{C}(\varepsilon_1',\varepsilon_1|\mX) \tag{Since $\mathbb{C}(\varepsilon_i', \varepsilon_j|\mX) = 0 ~ \forall i \neq j$}
%& = \mathbb{C}\big(\varepsilon_1',  \sum_{j=1}^d \sum_{k=1}^d x_{1j}' h_{jk} \big( \sum_{i=1}^n x_{ik} \varepsilon_i \big)|\mX \big) \\
%& = \mathbb{C}(\varepsilon_1', h(\varepsilon_1, \dots, \varepsilon_n)|\mX) \tag{$h(\varepsilon_1, \dots, \varepsilon_n) := \mX_1'^\top (\mX^\top \mX)^{-1} \mX^\top \vm{\varepsilon}$}.
%&=  \mathbb{C}(\varepsilon_1', \mX_1'^\top H x_1 \varepsilon_1) \\
%&=  \mathbb{C}(\varepsilon_1', \varepsilon_1) \cdot  \mX_1'^\top H x_1,
\end{align}
% Here, we can either invoke Stein's Lemma, or we can realize that $\varepsilon_1'$ and $\varepsilon_i$ only co-vary for the training data index $i=1$. Thus, we obtain:
% \begin{align}
% \mathbb{C}(y_1', \btheta^\top \mX_1'|\mX) & = \mathbb{C}\big(\varepsilon_1',  \sum_{j=1}^d \sum_{k=1}^d x_{1j}' h_{jk} (x_{1k} \varepsilon_1 + \sum_{i=2}^n x_{ik} \varepsilon_i)|\mX \big) \\
%  & = \mathbb{C}\big(\varepsilon_1', \varepsilon_1 \sum_{j=1}^d \sum_{k=1}^d x_{1j}' h_{jk} x_{1k}|\mX\big) \tag{Since $\mathbb{C}(\varepsilon_i', \varepsilon_j|\mX) = 0 ~ \forall i \neq j$} \\
%  &=  \mathbb{C}(\varepsilon_1', \varepsilon_1|\mX) \cdot  \mX_1'^\top (\mX^\top \mX)^{-1} \mX_1,
% \end{align}
where $\mX_1 \in \mathcal{D}_{\text{Train}}$.
Note, that when the null hypothesis is true (i.e., $\mX_1' \neq \mX_1 \in \mathcal{D}_{\text{Train}}$), we have:
\begin{align}
\mathbb{C}(y_1', \btheta^\top \mX_1'|\mX, \bz_1' \not \in \mathcal{D}_{\text{Train}}) &=  \mathbb{C}(\varepsilon_1', \varepsilon_1|\mX,\bz_1' \not \in \mathcal{D}_{\text{Train}}) \\
&= 0,
\end{align}
on the other hand: when the alternative is true, we have:
\begin{align}
\mathbb{C}(y_1', \btheta^\top \mX_1'|\mX, \bz_1' \in \mathcal{D}_{\text{Train}}) &= \mathbb{C}(\varepsilon_1', \varepsilon_1|\mX,\bz_1' \in \mathcal{D}_{\text{Train}}) \\
& = \mathbb{V}(\varepsilon_1 |\mX,\bz_1' \in \mathcal{D}_{\text{Train}}) \\
& =  \sigma^2.
\end{align}

Thus, from this it follows that the loss follows different Gaussians depending on the hypothesis we are under:
\begin{align}
\text{H}_0 (\bz_1' \in \mathcal{D}_{\text{Train}}) &: y_1' - \btheta^\top \mX_1' \sim \mathcal{N}\big(0, \sigma^2 - \sigma^2  \mX_1'^\top (\mX^\top \mX)^{-1} \mX_1'\big) \label{eq:h1_gaussian}\\
\text{H}_1 (\bz_1' \not \in \mathcal{D}_{\text{Train}}) &: y_1' - \btheta^\top \mX_1' \sim \mathcal{N}\big(0, \sigma^2 + \sigma^2 \mX_1'^\top (\mX^\top \mX)^{-1} \mX_1' \big) \label{eq:ho_gaussian} 
\end{align}
In other words, we are testing differences in variances of the losses. 
%Next, recall the following fact pertaining to the relation between Gaussian and Chi-squared distributions.
%Let $A \sim \mathcal{N}(0, \sigma^2)$. Then $A^2 \sim \sigma^2 \mathcal{X}^2(1)$.
%Thus, it readily follows that:
%\begin{align}
%    \Lambda_{loss} = \frac{\sigma^2 + \mX_1'^\top H \mX_1'}{\sigma^2 + \mX_1'^\top H \mX_1' - 2 \cdot \mX_1'^\top H x_1 \cdot \sigma^2} > \tau.
%\end{align}
Let's denote the variances under $H_0$ and $H_1$ by $v_0:=\sigma^2 \cdot \big(1 - \mX_1'^\top (\mX^\top \mX)^{-1} \mX_1' \big)$ and $v_1:=\sigma^2 \cdot \big(1 + \mX_1'^\top (\mX^\top \mX)^{-1} \mX_1'\big)$, respectively.
Then, using the Gaussian likelihoods from \eqref{eq:ho_gaussian} and \eqref{eq:h1_gaussian} the likelihood-ratio in favour of $H_1$ can be written as follows:
\begin{align}
\Lambda_{\text{Loss}} = \sqrt{\frac{v_1}{v_0}} \exp \bigg( - (y_1' - \btheta \mX_1')^2 \bigg( \frac{1}{2v_0} - \frac{1}{2v_1} \bigg) \bigg) \geq \tau.
\end{align}

\paragraph{Rewriting the LRT in terms of the Loss-Statistic}
Note that $v_0 < v_1$ and for $v_0 < v_1$, rearranging the terms yields that we reject $H_0$ (i.e., train set membership) in favour of $H_1$ (not in train set) if (the loss is large):
\begin{align}
\ell = (y_1' - \btheta \mX_1')^2 \geq  \gamma := 2 \bigg( \frac{v_0 v_1}{v_1 - v_0} \bigg) \bigg( \log(\tau) + \log\bigg(\frac{v_1}{v_0}\bigg) \bigg) \geq 0.
\end{align}
Next, note that the distributions under both hypotheses can be rewritten as follows ($\nu_0$ and $\nu_1$ known):
\begin{align}
\text{H}_0 (\bz_1' \in \mathcal{D}_{\text{Train}}) &:  T_0 = \frac{(y_1' - \btheta^\top \mX_1')^2}{v_0} \sim \mathcal{X}^2(1) \\
\text{H}_1 (\bz_1' \not \in \mathcal{D}_{\text{Train}}) &:  T_1 = \frac{(y_1' - \btheta^\top \mX_1')^2}{v_1} \sim \mathcal{X}^2(1).
\end{align}

\paragraph{Determining the Theoretical Power and Size of the Test}
Next, our goal is to find the false-positive rate (also called the `size') and the true positive rate (also called the statistical `power') of the LRT in terms of $\gamma$.
Thus, the false positive rate is given by:
\begin{align}
p_{\text{FPR}} &= \int^{\infty}_{\gamma} p_0(x) dx \\
              &= \mathbb{P}_{\ell \sim p_0}(\ell \geq \gamma) \\
              &= 1 - \mathbb{P}_{\ell \sim p_0}\bigg(\frac{\ell}{\nu_0} \leq \frac{\gamma}{\nu_0} \bigg) \\
              &= 1 - \mathbb{P}_{\mathcal{X}^2_1}\bigg(T_0 \leq \frac{\gamma}{\nu_0} \bigg) \\
              &= 1 - \text{CDF}_{\mathcal{X}^2_1}\bigg(\frac{\gamma}{v_0}\bigg),
\end{align}
while the true positive rate (power) is defined as:
\begin{align}
    p_{\text{TPR}} &= \int^{\infty}_{\gamma} p_1(x) dx \\
                     &= \mathbb{P}_{\ell^2 \sim p_1}(v_1 T_1 \geq \gamma) \\
                     &= 1 - \mathbb{P}_{\ell^2 \sim p_1}(v_1 T_1 \leq \gamma) \\
                     &= 1- \text{CDF}_{\mathcal{X}^2_1}\bigg(\frac{\gamma}{v_1}\bigg).
\end{align}
Now, for a given $p_{\text{FPR}}=\alpha$, we can compute $\gamma^*$ in terms of $\alpha$ and $v_0$ since the CDF is invertible:
\begin{align}
    \gamma^* = v_0 \text{CDF}_{\mathcal{X}^2_1}^{-1} \big( 1 - \alpha \big).
\end{align}
Next, plugging $\gamma^*$ into $p_{\text{TPR}}$ we obtain the optimal power at fixed false-positive-rate $\alpha$:
\begin{align}
    p_{\text{TPR}} = \text{CDF}_{\mathcal{X}^2_1}\bigg(\frac{v_0}{v_1} \text{CDF}_{\mathcal{X}^2_1}^{-1} \big(1-  \alpha \big)\bigg).
\end{align}
Thus, when $v_0$ is large relative to $v_1$ the LRT will have high power! This completes our proof.
%Note that this is also intuitive; see the Figure above. 
\end{proof}

\subsection{Observations}
Note the following:
While FPR is being fixed, and TPR is being maximized, from a practical point of view, we do not care about them!
We care more about TNR (i.e., say $z$ is train member when it is) and the FNR (i.e., we want to control: when $z$ is not a train member say that at most $\alpha \times 100$ times):
\begin{align}
p_{\text{TNR}} &= \int_{-\infty}^{\gamma} p_0(x) dx = \text{CDF}_{\mathcal{X}^2_1}\bigg(\frac{\gamma}{v_0}\bigg)  \\
p_{\text{FNR}} &= \int_{-\infty}^{\gamma} p_1(x) dx =  1 - \text{CDF}_{\mathcal{X}^2_1}\bigg(\frac{v_0}{v_1} \text{CDF}_{\mathcal{X}^2_1}^{-1} \big(1-  \alpha \big)\bigg). 
\end{align}

==> 5-GaussianMechanismPrivacy.tex <==
% \section{Relating Membership Inference and Differential Privacy for Mean Estimation with Gaussian Mechanisms}

% While differentially private algorithms can be obtained in different ways, randomness needs to be involved in all differentially private processes.


% \begin{definition}
% For a function $f: \mathbb{R}^k \rightarrow \mathbb{R}^d$, and input $X \in \mathbb{R}^k$, the Gaussian mechanism $M:\mathbb{R}^k \rightarrow \mathbb{R}^d$ is defined as 
% \begin{align}
%     M(X) = f(X) + Y,
% \end{align}
% where $Y\in \mathbb{R}^{d}$ follows a Gaussian distribution with $Y \sim \mathcal{N}(\mathbf{0}, \tau^2\mI)$.
% \end{definition}

% \subsection{How does the Gaussian Mechanism affect $\mu_{\text{MIP}}$-privacy}
% In this section, we study how the common Gaussian mechanism affects attack accuracy in terms of $\mu$-privacy. With the specific attack model incorporated in two distribution $P$, $Q$, $\mu$-Privacy is fulfilled when the attacker cannot separate $P$ and $Q$ better than given by the trade-off curve:
% \begin{align}
% \beta = \Phi(\Phi^{-1}(1-\alpha)-\mu).
% \end{align}
% \textbf{Differential Privacy.} We restate the following theorem, which provides insights on how the Gaussian mechanism results in $\mu$-Gaussian Differential Privacy.
% \begin{theorem}[Theorem 2.7 from \cite{dong2022gaussian}]
% Define the Gaussian mechanism that operates on a statistic $f(S)$ defined  as $M(S) = f(S)+Y$,
% where $Y \sim \mathcal{N}\left(\mathbf{0}, \frac{\lVert f\rVert_2^2}{\mu_G^2} \mI\right)$. In this notation, $\lVert f\rVert_2$ denotes the sensitivity of $f$ with respect to the $l_2$-norm. Then $M(S)$ is $\mu_G$-private.
% \end{theorem}


%\subsection{Testing with added unit noise}


%$$
% \begin{align}
% \vm-\vx^{'}-Y \sim \mathcal{N}\left(0, \frac{n-1}{n}\mSigma + \tau^2 \mI \right).
% \end{align}
% Thus, the test statistic under the null hypothesis is given by:
% \begin{align}
% S_0 = (\vm - \vx^{'} - Y)^\top \left(\frac{n-1}{n}\mSigma +\tau^2\mI \right)^{-1}(\vm - \vx^{'} - Y)\sim \chi^2(d).
% \end{align}
% For now, we consider the simplified version where $\mSigma = \mI$, in which case:
% \begin{align}
% S_0 & = (\vm - \vx^{'} - Y)^\top \left(\frac{n-1}{n}\mI +\tau^2\mI \right)^{-1}(\vm - \vx^{'} - Y)\sim \chi^2(d) \\
% &= (\vm - \vx^{'} - Y)^\top \left(\frac{(1 + \tau^2) n - 1}{n} \right)^{-1}(\vm - \vx^{'} - Y)\sim \chi^2(d) \\
% &= \left(\frac{n}{(1 + \tau^2) n - 1} \right)  (\vm - \vx^{'} - Y)^\top (\vm - \vx^{'} - Y)\sim \chi^2(d).
% \end{align}

% The probability of accepting the hypothesis is given as
% %\begin{align}
% %    \beta = & P\left(\frac{n}{n-1} (\vm %- \vx^{'})^\top \mSigma^{-1} (\vm - %\vx^{'}) \leq %\text{CDF}_{\mathcal{X}^2_d}^{-1}
    
% Under the alternative Hypotheses $H_1$ we have:
% \begin{align}
% S_1 = \vm-\vx^{'}-Y \sim \mathcal{N}\left(0, \frac{n+1}{n}\mSigma + \tau^2 \mI \right)
% \end{align}
% The test statistic follows the distribution:
% \begin{align*}
% (\vm - \vx^{'} - Y)^\top \left(\frac{n+1}{n}\mSigma +\tau^2\mI \right)^{-1}(\vm - \vx^{'} - Y)\sim \chi^2(d).
% \end{align*}
% For now, we consider the simplified version where $\mSigma = \mI$, in which case:
% \begin{align*}
% S_1 & = (\vm - \vx^{'} - Y)^\top \left(\frac{n+1}{n}\mI +\tau^2\mI \right)^{-1}(\vm - \vx^{'} - Y)\sim \chi^2(d) \\
% &= \left(\frac{n}{1 + (1 + \tau^2) n} \right) (\vm - \vx^{'} - Y)^\top (\vm - \vx^{'} - Y)\sim \chi^2(d) 
% \end{align*}

% \begin{align}
% \mu_{\text{MIP}} = \frac{2d + \frac{(3n - 1) K}{1+\tau^2} }{(n+1)\sqrt{2d + 4 n \frac{K}{1+\tau^2} }}.
% \end{align}
